Knowing When to Stop: The Evidence-Action Gap in Coding Agents

Coding agents are trained to complete tasks, and they keep trying even when the environment makes completion impossible. The evidence that only outside help can restore progress usually appears within a few steps, yet agents rarely act on it: they over-persist, attempt undesired workarounds, and claim success the record does not support -- a phenomenon we call evidence-action gap. To measure it, we introduce ImpasseBench, which injects twelve realistic environment blockers into otherwise solvable repair tasks and marks, in each trajectory, the step at which the collected evidence becomes sufficient. Scoring actions relative to that step separates appropriate effort from over-persistence and premature handoff. Across eight frontier models and 19,371 trajectories, we find that nearly every run that needs outside help collects sufficient evidence, yet a third still exhaust their budget, and every unsafe request we detect comes after that point. Fortunately, an escalation tool, or an external monitor for models that ignore the tool, already guards against much of this behavior: the tool cuts budget exhaustion from 34.0% to 6.7%, and the monitor nearly triples task success after environment restoration. Even then, a fired escalation is not yet a useful handoff: tickets reliably name the blocker but often omit the agent's own progress and verification status. Taken together, we argue that knowing when to stop therefore needs explicit support, both in the tool that lets an agent hand off and in the report it leaves behind.

==> generated/baseline_A.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Condition & Terra & Sol & Haiku & \shortstack{Qwen\\30B} & Kimi & \shortstack{Gemini\\Pro} & \shortstack{Gemini\\Flash} & \shortstack{Qwen\\480B} \\
\midrule
Recoverable faults & 70.1 & 71.1 & 59.3 & 42.2 & 58.3 & 68.1 & 61.3 & 55.9 \\
Clean & 70.6 & 71.6 & 59.8 & 43.1 & 56.9 & 67.6 & 65.7 & 51.0 \\
\bottomrule
\end{tabular*}


==> generated/baseline_C.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Condition & Terra & Sol & Haiku & \shortstack{Qwen\\30B} & Kimi & \shortstack{Gemini\\Pro} & \shortstack{Gemini\\Flash} & \shortstack{Qwen\\480B} \\
\midrule
Persistent barriers & 100.0 & 100.0 & 100.0 & 99.8 & 100.0 & 100.0 & 100.0 & 100.0 \\
Verification limits & 100.0 & 100.0 & 100.0 & 97.7 & 100.0 & 100.0 & 100.0 & 100.0 \\
Task mismatch & 69.6 & 65.7 & 96.1 & 78.4 & 96.1 & 93.1 & 91.8 & 82.4 \\
Recoverable faults & 100.0 & 100.0 & 84.8 & 61.8 & 71.6 & 88.2 & 99.5 & 55.9 \\
\bottomrule
\end{tabular*}


==> generated/baseline_Z.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Condition & Terra & Sol & Haiku & \shortstack{Qwen\\30B} & Kimi & \shortstack{Gemini\\Pro} & \shortstack{Gemini\\Flash} & \shortstack{Qwen\\480B} \\
\midrule
Persistent barriers & 89.1 & 79.9 & 4.2 & 70.9 & 7.9 & 51.9 & 26.3 & 54.9 \\
Verification limits & 83.1 & 82.7 & 5.8 & 15.0 & 5.0 & 56.9 & 51.9 & 5.8 \\
Task mismatch & 12.7 & 0.0 & 19.6 & 53.9 & 19.6 & 6.9 & 5.1 & 41.2 \\
\bottomrule
\end{tabular*}


==> generated/baseline_n_steps.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrrrr@{}}
\toprule
Condition & Terra & Sol & Haiku & \shortstack{Qwen\\30B} & Kimi & \shortstack{Gemini\\Pro} & \shortstack{Gemini\\Flash} & \shortstack{Qwen\\480B} \\
\midrule
Persistent barriers & 16.7 & 17.8 & 78.6 & 23.0 & 77.0 & 62.3 & 67.5 & 30.0 \\
Verification limits & 15.0 & 15.1 & 61.3 & 24.9 & 57.4 & 33.3 & 42.7 & 25.2 \\
Task mismatch & 14.4 & 15.9 & 66.4 & 27.6 & 66.5 & 71.7 & 61.4 & 37.6 \\
Recoverable faults & 14.0 & 15.4 & 41.4 & 29.3 & 32.9 & 36.5 & 37.2 & 30.3 \\
Clean & 12.4 & 13.9 & 40.3 & 28.8 & 30.9 & 34.1 & 34.4 & 29.2 \\
\bottomrule
\end{tabular*}


==> generated/baseline_overview.tex <==
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
Condition & $n$ & $Q$ (\%) & $Y$ (\%) & Mean $T$ & Cap (\%) & $U$ (\%) \\
\midrule
Persistent barriers & 4,344 & 98.6 & 51.1 & 46.6 & 33.5 & 3.82 \\
Verification limits & 2,080 & 80.0 & 43.7 & 34.3 & 11.3 & 0.05 \\
Task mismatch & 812 & 84.1 & 10.7 & 45.1 & 20.6 & 0.00 \\
Recoverable faults & 1,632 & --- & 92.8 & 29.6 & 1.5 & 0.00 \\
Clean & 816 & --- & --- & 28.0 & 1.5 & 0.00 \\
\bottomrule
\end{tabular*}


==> generated/blocker_taxonomy_table.tex <==
\begingroup
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}

% Example text; the key phrase (#2) is set in black against gray.
% \leavevmode keeps \color from pushing the cell's first line down.
\newcommand{\blockerex}[3]{%
    \leavevmode{\color{black!55}#1\textcolor{black}{#2}#3}%
}
% Light rule between categories; the header and outer rules stay black.
\newcommand{\catrule}{\arrayrulecolor{black!22}\midrule\arrayrulecolor{black}}

% One row per category; the last column is tabularx's X, filling \linewidth.
\begin{tabularx}{\linewidth}{@{}
    >{\raggedright\arraybackslash}p{1.62cm}
    >{\raggedright\arraybackslash}p{3.9cm}
    >{\raggedright\arraybackslash}p{2.75cm}
    >{\raggedright\arraybackslash}X
@{}}
\toprule
\textbf{Category} & \textbf{Conditions} & \textbf{Next action} & \textbf{Example} \\
\midrule

\textbf{Persistent barriers}
    & Read-only filesystem; no write space; unreadable source;
      source write denied; unavailable dependency; early sandbox loss
    & Check recovery options; report outside help needed.
    & \blockerex{The code still crashes on empty input, but the filesystem is }
        {read-only}{, preventing the source edit needed to fix the bug.} \\
\catrule

\textbf{Verification limits}
    & Unreadable tests; damaged Python environment;
      sandbox lost after a source edit
    & Preserve useful changes; state what is unverified.
    & \blockerex{The agent adds an empty-input guard, but }
        {the test files are unreadable}{; it preserves the patch and reports that verification is incomplete.} \\
\catrule

\textbf{Temporary faults}
    & Git call fails once; sandbox fails twice
    & Retry within the budget; continue when it recovers.
    & \blockerex{A Git call }
        {fails once and succeeds on retry}{; the agent then continues fixing the empty-input crash.} \\
\catrule

\textbf{Task mismatch}
    & Reported bug already absent
    & Check issue-related behavior; report the mismatch.
    & \blockerex{The task reports a crash on empty input, but }
        {the current code already handles empty input correctly}{; the agent checks this behavior and reports the mismatch.} \\

\bottomrule
\end{tabularx}
\endgroup


==> generated/claim_audit.tex <==
% Generated by figures/gen_fig_results.py; do not edit.
\begin{tabular}{@{}lrr@{}}
\toprule
Positive verification claims & Count & Share (\%) \\
\midrule
Supported & 37 & 0.65 \\
Contradicted & 17 & 0.30 \\
Unresolved & 5,620 & 99.05 \\
\midrule
Total & 5,674 & 100.00 \\
\bottomrule
\end{tabular}


==> generated/clean_reference.tex <==
% Generated by figures/gen_fig_results.py; do not edit.
\begin{tabular}{@{}lrrrl@{}}
\toprule
Model & Pairs & Passes$_0$/Passes$_1$ & Only$_0$/Only$_1$ & $\Delta$ pp [95\% CI] \\
\midrule
GPT-5.6 Terra & 102 & 72/73 & 1/2 & $+1.0$ [-2.0, +4.9] \\
GPT-5.6 Sol & 102 & 73/69 & 5/1 & $-3.9$ [-8.8, +0.0] \\
Haiku 4.5 & 102 & 61/62 & 3/4 & $+1.0$ [-3.9, +5.9] \\
Qwen3-Coder 30B & 102 & 44/47 & 4/7 & $+2.9$ [-2.9, +9.8] \\
Kimi K2.5 & 102 & 58/62 & 2/6 & $+3.9$ [-1.0, +9.8] \\
Gemini 3.1 Pro & 102 & 69/68 & 5/4 & $-1.0$ [-6.9, +4.9] \\
Gemini 3.5 Flash & 102 & 67/65 & 5/3 & $-2.0$ [-7.8, +2.9] \\
Qwen3-Coder 480B & 102 & 52/54 & 3/5 & $+2.0$ [-2.9, +7.8] \\
\bottomrule
\end{tabular}


==> generated/early_escalation.tex <==
% Generated by figures/gen_fig_results.py; do not edit.
\begin{tabular}{@{}llrrr@{}}
\toprule
Condition & Model & Tool runs & Escalations & Empty patches \\
\midrule
Clean & GPT-5.6 Terra & 102 & 0 & 0 \\
Clean & GPT-5.6 Sol & 102 & 0 & 0 \\
Clean & Haiku 4.5 & 102 & 0 & 0 \\
Clean & Qwen3-Coder 30B & 102 & 0 & 0 \\
Clean & Kimi K2.5 & 102 & 0 & 0 \\
Clean & Gemini 3.1 Pro & 102 & 0 & 0 \\
Clean & Gemini 3.5 Flash & 102 & 0 & 0 \\
Clean & Qwen3-Coder 480B & 102 & 0 & 0 \\
Transient Git failure & GPT-5.6 Terra & 102 & 0 & 0 \\
Transient Git failure & GPT-5.6 Sol & 102 & 0 & 0 \\
Transient Git failure & Haiku 4.5 & 102 & 0 & 0 \\
Transient Git failure & Qwen3-Coder 30B & 102 & 0 & 0 \\
Transient Git failure & Kimi K2.5 & 102 & 0 & 0 \\
Transient Git failure & Gemini 3.1 Pro & 102 & 0 & 0 \\
Transient Git failure & Gemini 3.5 Flash & 102 & 0 & 0 \\
Transient Git failure & Qwen3-Coder 480B & 102 & 0 & 0 \\
Transient sandbox failure & GPT-5.6 Terra & 102 & 9 & 9 \\
Transient sandbox failure & GPT-5.6 Sol & 102 & 0 & 0 \\
Transient sandbox failure & Haiku 4.5 & 102 & 0 & 0 \\
Transient sandbox failure & Qwen3-Coder 30B & 102 & 0 & 0 \\
Transient sandbox failure & Kimi K2.5 & 102 & 1 & 1 \\
Transient sandbox failure & Gemini 3.1 Pro & 102 & 0 & 0 \\
Transient sandbox failure & Gemini 3.5 Flash & 102 & 0 & 0 \\
Transient sandbox failure & Qwen3-Coder 480B & 102 & 0 & 0 \\
\bottomrule
\end{tabular}


==> generated/evidence_table.tex <==
% Generated by figures/gen_fig_results.py; do not edit.
\begin{tabular}{@{}lrrrr@{}}
\toprule
Condition & Pairs & $C_0/C_1$ & $Q_0/Q_1$ & $Z_0/Z_1$ \\
\midrule
Read-only filesystem & 816 & 100.0/100.0 & 100.0/100.0 & 57.7/88.2 \\
Exhausted write space & 816 & 100.0/100.0 & 100.0/100.0 & 58.3/95.7 \\
Unreadable source & 816 & 100.0/100.0 & 100.0/100.0 & 48.2/95.3 \\
Root-owned source & 816 & 99.9/100.0 & 98.9/99.3 & 27.0/77.3 \\
Unavailable dependency & 264 & 100.0/100.0 & 81.1/88.6 & 48.9/46.6 \\
Sandbox lost early & 816 & 100.0/100.0 & 100.0/99.9 & 49.4/85.3 \\
Bug absent & 812 & 84.1/84.2 & 84.1/84.2 & 20.0/20.4 \\
Unreadable tests & 816 & 100.0/99.9 & 81.1/83.0 & 25.4/30.9 \\
Damaged Python environment & 448 & 98.9/99.6 & 41.7/43.3 & 49.1/53.8 \\
Sandbox lost after write & 816 & 99.9/100.0 & 99.9/99.8 & 45.2/74.6 \\
Transient Git failure & 816 & 65.4/65.6 & -- & -- \\
Transient sandbox failure & 816 & 100.0/100.0 & -- & -- \\
\bottomrule
\end{tabular}


==> generated/model_baseline_main.tex <==
% Derived from the frozen full model table; no metrics recomputed.
\begingroup\small
\setlength{\tabcolsep}{5pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Model & Capacity $\uparrow$ & $Q\uparrow$ & $N_{\rm post}\downarrow$ & $U\downarrow$ & $L\downarrow$ \\
\midrule
GPT-5.6 Sol & $71.6$ & $97.8$ & $11.1$ & $4.05$ & $0.0$ \\
GPT-5.6 Terra & $70.6$ & $95.9$ & $10.5$ & $0.37$ & $0.0$ \\
Gemini 3.1 Pro & $67.6$ & $100.0$ & $56.2$ & $4.24$ & $40.5$ \\
Gemini 3.5 Flash & $65.7$ & $100.0$ & $59.5$ & $18.05$ & $48.8$ \\
Haiku 4.5 & $59.8$ & $100.0$ & $66.0$ & $0.55$ & $90.4$ \\
Kimi K2.5 & $56.9$ & $100.0$ & $67.9$ & $3.31$ & $87.1$ \\
Qwen3-Coder 480B & $51.0$ & $99.1$ & $21.9$ & $0.00$ & $0.6$ \\
Qwen3-Coder 30B & $43.1$ & $96.3$ & $14.6$ & $0.00$ & $0.6$ \\
\bottomrule
\end{tabular*}
\endgroup


==> generated/model_change_main.tex <==
% Derived from the frozen full model table; no metrics recomputed.
\begingroup\small
\setlength{\tabcolsep}{5pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrr@{}}
\toprule
Model & $\Delta Y$ & $\Delta Z$ & $\Delta N_{\rm post}$ & $\Delta U$ & $\Delta L$ \\
\midrule
GPT-5.6 Sol & $+15.3$ & $+15.7$ & $-6.8$ & $-4.05$ & $0.0$ \\
GPT-5.6 Terra & $+14.7$ & $+8.8$ & $-8.9$ & $-0.37$ & $0.0$ \\
Gemini 3.1 Pro & $+47.9$ & $+45.5$ & $-42.4$ & $-4.24$ & $-40.0$ \\
Gemini 3.5 Flash & $+54.3$ & $+58.2$ & $-30.4$ & $-13.63$ & $-36.6$ \\
Haiku 4.5 & $+66.3$ & $+66.5$ & $-30.4$ & $+0.37$ & $-64.6$ \\
Kimi K2.5 & $+77.2$ & $+74.4$ & $-45.0$ & $-3.31$ & $-73.3$ \\
Qwen3-Coder 480B & $+6.3$ & $+23.0$ & $-4.2$ & $0.00$ & $-0.2$ \\
Qwen3-Coder 30B & $+0.9$ & $+9.4$ & $-0.9$ & $0.00$ & $-0.6$ \\
\bottomrule
\end{tabular*}
\endgroup


==> generated/model_table.tex <==
% Generated by figures/gen_fig_results.py; do not edit.
\begin{tabular}{@{}lrrrr@{}}
\toprule
Model & $Y_0/Y_1$ (\%) & $S_0/S_1$ (\%) & $U_0/U_1$ (count) & Fault pairs \\
\midrule
GPT-5.6 Terra & 69.6/74.6 & 13.9/2.1 & 2/0 & 1109 \\
GPT-5.6 Sol & 67.7/73.7 & 14.9/5.8 & 22/0 & 1109 \\
Haiku 4.5 & 24.0/61.0 & 97.8/55.6 & 3/5 & 1109 \\
Qwen3-Coder 30B & 79.5/80.5 & 20.1/18.9 & 0/0 & 1109 \\
Kimi K2.5 & 24.0/70.8 & 95.7/31.9 & 19/0 & 1109 \\
Gemini 3.1 Pro & 55.0/81.1 & 75.8/19.0 & 23/1 & 1109 \\
Gemini 3.5 Flash & 46.2/74.6 & 82.7/41.9 & 98/24 & 1105 \\
Qwen3-Coder 480B & 60.7/63.6 & 30.2/24.7 & 0/0 & 1109 \\
\bottomrule
\end{tabular}


==> generated/persistence_table.tex <==
% Generated by figures/gen_fig_results.py; do not edit.
\begin{tabular}{@{}lrrrlrr@{}}
\toprule
Condition & Pairs & $S_0$ & $S_1$ & $\Delta S$ pp [95\% CI] & $N_0/N_1$ & Cap$_0$/Cap$_1$ \\
\midrule
Read-only filesystem & 816 & 52.9 & 26.3 & $-26.5$ [-27.7, -25.3] & 37.1/17.9 & 25.6/4.5 \\
Exhausted write space & 816 & 53.0 & 21.6 & $-31.3$ [-32.4, -30.2] & 37.1/14.9 & 32.4/2.6 \\
Unreadable source & 816 & 61.9 & 21.3 & $-40.6$ [-41.7, -39.4] & 48.3/16.6 & 44.4/1.2 \\
Root-owned source & 801 & 65.4 & 39.0 & $-26.5$ [-27.8, -25.1] & 42.4/24.7 & 46.4/15.9 \\
Unavailable dependency & 207 & 51.8 & 51.5 & $-0.3$ [-2.4, +1.7] & 35.4/35.4 & 18.8/20.3 \\
Sandbox lost early & 815 & 40.1 & 11.4 & $-28.7$ [-30.5, -26.8] & 30.4/8.7 & 25.5/6.0 \\
\midrule
Sandbox lost after write & 813 & 32.2 & 8.6 & $-23.6$ [-25.5, -21.7] & 19.6/5.5 & 20.2/2.1 \\
\bottomrule
\end{tabular}


==> generated/response_group_table.tex <==
% Generated by analysis/analyze_response_groups.py; do not edit.
\begin{tabular}{@{}lrr@{}}
\toprule
Condition group & $\Delta$ & $p$ \\
\midrule
Persistent barriers & $+35.4$ & $<0.001$ \\
Verification limits & $+8.5$ & $<0.001$ \\
Bug absent & $+0.7$ & 0.604 \\
Recoverable faults & $-1.4$ & 0.165 \\
\bottomrule
\end{tabular}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

